Deterministic Browser

Timing attacks have been a continuous threat to users' privacy in modern browsers. To mitigate such attacks, existing approaches, such as Tor Browser and Fermata, add jitters to the browser clock so that an attacker cannot accurately measure an event. However, such defenses only raise the bar for an attacker but do not fundamentally mitigate timing attacks, i.e., it just takes longer than previous to launch a timing attack. In this paper, we propose a novel approach, called deterministic browser, which can provably prevent timing attacks in modern browsers. Borrowing from Physics, we introduce several concepts, such as an observer and a reference frame. Specifically, a snippet of JavaScript, i.e., an observer in JavaScript reference frame, will always obtain the same, fixed timing information so that timing attacks are prevented; at contrast, a user, i.e., an oracle observer, will perceive the JavaScript differently and do not experience the performance slowdown. We have implemented a prototype called DeterFox and our evaluation shows that the prototype can defend against browser-related timing attacks.

==> Makefile <==
# $Id: Makefile,v 1.1 2013/07/13 00:34:30 yzcao Exp $

LATEX=pdflatex
BIBTEX = bibtex

PAPER=main

BIBFILE = replicate
	
PS2PDF = ps2pdf -dPDFSETTINGS=/prepress -dMaxSubsetPct=100 -dCompatibilityLevel=1.4 -dSubsetFonts=true -dEmbedAllFonts=true
MKPDF = myps2pdf

TEXFILES = \
	*.tex \

all: $(PAPER).pdf
#$(PAPER).ps $(PAPER).pdf
#	gawk -f degunk.awk $(PAPER).ps > tmp.ps
#	mv tmp.ps $(PAPER).ps

$(PAPER).pdf:
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)

$(PAPER).ps: $(PAPER).dvi
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)

$(PAPER).dvi: $(FIGS) $(TEXFILES)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)

$(PREPRINT).ps: $(PREPRINT).dvi
	dvips -P cmz -t letter -f $(PREPRINT).dvi > $(PREPRINT).ps

$(PREPRINT).dvi: $(FIGS) $(TEXFILES) $(PREPRINT).tex
	$(LATEX) $(PREPRINT)
	$(LATEX) $(PREPRINT)

%.pdf: %.ps

clean:
	/bin/rm -f main.pdf *.dvi *.aux main.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl

tarball:
	rm -f imc.tar.gz
	tar -cf imc.tar Makefile todo IEEE.bst sig-alternate.cls *.sty \
		*.tex *.bib virtualy.* imc.ps figures/*
	gzip imc.tar

loop:
	latexmk -pvc -view=pdf -pdflatex='pdflatex -file-line-error -synctex=1' main.tex

# Manuel cmdline: latexmk -pvc -view=pdf -pdflatex='pdflatex -file-line-error -synctex=1' main.tex



==> back.tex <==
Note that there is an interesting property of a deterministic reference frame, i.e., when the same $RF$ is executed twice, if an $Ob$ makes the same observation ($O^{E1}$ and $O^{E2}$) in these two $RF$s, the difference of the timestamps ($t^{E1}_{Ob}$ and $t^{E2}_{Ob}$) of the two observations is only related to  the starting timestamps ($t^{E1}_{St}$ and $t^{E2}_{St}$) of the $RF$s.


\begin{equation}
\begin{split}
&t^{E1}_{Ob} - t^{E2}_{Ob} = (t^{E1}_{Ob} - t^{E1}_{St}) - (t^{E2}_{Ob} - t^{E2}_{St}) + t^{E1}_{St} - t^{E2}_{St} \\
&= f(O^{E1}, O^{E1}_{St}, RF) - f(O^{E1}, O^{E1}_{St}, RF) + t^{E1}_{St} - t^{E2}_{St} \\
&= t^{E1}_{St} - t^{E2}_{St}
\end{split}
\end{equation}


\begin{definition}
Given a set of opcodes ($SO$) generated from a program, a fixed initial state, and a set of fixed inputs ($I$) happening at fixed timestamps, {\bf strong determinism} defines that for different executions on different environments, at time $t$, the same opcode ($op$) will be executed and the same outputs ($O_{op, I}$) will be produced.  

%for each execution, each opcode ($op$) in $JO$ will produce exactly the same outputs ($O_{op, I}$)
\end{definition}


Strong determinism states that when inputs for a browser are fixed, every JavaScript operation will produce the same results at the same timestamp in different environments. That is, when a snippet of JavaScript tries to fingerprint the environment that it is executing upon, the JavaScript cannot differentiate the environments as they look exactly the same from the viewpoint of the JavaScript. 


Strong determinism can defend browser fingerprinting, however it assumes that every execution starts at the same timestamp---being unrealistic for modern browsers because in real world the time elapses and never comes back.  Therefore, we propose weak determinism, a variance of strong determinism but taking different starting timestamps into consideration.  




The concept of reference frame, borrowed from Physics, consists of ``an abstract coordinate system and the set of physical reference points that uniquely fix the coordinate system and standardize measurements.'' In the context of deterministic browser, a reference frame is one-dimension  system and consists of only time. The measurement of time is performed by {\it clocks}, which ticks based on certain criteria, such as the physical clock, the execution of an opcode, and the invocation of a document object model (DOM) method. 

We further classify reference frames into two major categories: main and auxiliary.  A main reference frame has an {\it observer}, a Turing complete program, e.g., capable of fingerprinting the runtime environment; an auxiliary reference frame does not have an observer. Correspondingly, we define a clock in a main reference frame as main clock, and a clock in auxiliary as auxiliary clock.  


%Below, we will show two auxiliary reference frame examples. 
A main reference frame can exist by itself; on the contrary, an auxiliary reference frame does not exist by itself, but is attached to a main reference frame.  That is, an auxiliary reference frame is created and destroyed by a main reference frame by operations.  
 For example, when a JavaScript sends a network request, a networking  auxiliary reference is created; when the JavaScript receives the response, the networking  auxiliary reference is created. 
 Lacking of observers, 
an auxiliary reference frame cannot fingerprint runtime environment, however it can convey information such as auxiliary clocks to the main  reference frame. 


Now, let us study the relationship between reference frames and determinism.  We say that a main reference frame is deterministic, if  the observer obeys the properties of determinism defined in Section~\ref{sec:def} under the clock of the reference frame.  That is, from the observer's viewpoint, the execution of opcodes distributed over time is in a fixed pattern, and the outputs of each opcode are only related to the starting time, initial state, and inputs.  

Because there are no observers in auxiliary reference frames, the determinism of an auxiliary reference frame is related to its parent main reference frame.  That is, if the operations of the observer in the parent reference frame---which interact with the auxiliary reference frame, such as creation and destroying---obeys the determinism properties under the clock of the auxiliary reference frame, the auxiliary reference frame is deterministic. 
%The reason is that

%determinism is undefined in auxiliary reference frames.


Below, we will take a look at some reference frame examples, how the clock ticks in these reference frames, and whether these reference frames are deterministic. \\ %, especially main reference frames to achieve determinism. \\

==> comp.tex <==
\section{Deterministic vs. Stochastic (Probabilistic)} \label{sec:vs}

Traditionally, there are two categories of approaches in defending browser fingerprinting: normalizing every fingerprint-able output (we call it deterministic output), and randomizing the output (we call it stochastic output).   However, neither approach is the key in defending fingerprinting.  Let us find the key.  Consider a fingerprint-able output as a random variable with the following distribution function:
\begin{equation}
f(o, x_1,x_2, ..., e) = Pr(O, X_1, X_2,..., E) 
\end{equation} 
where $o$ is the fingerprint-able output, $x_1$, $x_2$,..., are different parameters for the output, and $e$ is the runtime environment to generate the output.  For example, $f(Interval, op, E)$ is the probability of an opcode $op$ taking $Interval$ to execute in $E$; $f(Interval, IP, E)$ is the probability of a network request to $IP$ taking $Interval$ to finish in $E$; $f(Image, Inputs, E)$ is the probability of a canvas rendering an $Image$ with $Inputs$ in $E$. 

The reason of a fingerprint-able output $o$ is that $f(o, x_1,x_2, ..., E^1)$ and $f(o, x_1,x_2, ..., E^2)$ differ for $E^1$ and $E^2$. Based on the differences, one can recognize 
the corresponding $E$. For a simplified example, in $E^1$, an opcode $op$ has 0.5 probability to finish in 0.1ms, and 0.5 probability to finish in 0.2ms; at contrast, in $E^2$, an opcode $op$ has 0.5 probability to finish in 0.2ms, and 0.5 probability to finish in 0.3ms.  Based on average finishing time (0.15ms vs. 0.25ms), one can differentiate $E^1$ and $E^2$. 

Therefore, we believe that the key of defending fingerprinting lies in that the distribution functions for a fingerprint-able output are the same over different $E$s. That is, 
\begin{equation}
\forall E^1, \forall E^2, f(o, x_1,x_2, ..., E^1)=f(o, x_1,x_2, ..., E^2)
\end{equation}

Now, let us look back at deterministic and stochastic approaches.  Stochastic approach itself does not defend fingerprinting: Only when the distribution function for a stochastic output is deterministic, such approach can defend fingerprinting.  This is also the common mistake that existing approaches make in defending fingerprinting.  For example, Tor Browser~\cite{} adds jitters to $Date$ to defend JavaScript performance fingerprinting, however the browser can still be fingerprinted in a long run when the jitter is averaged out. Similarly, PriVaricator~\cite{} adds randomized noise to certain fingerprint-able outputs, however the browser can still be fingerprinted if one obtains the outputs many times and calculates the average. 

Deterministic approach can defend fingerprinting, because a deterministic output is a special case of stochastic approach with determined distribution function (at one point, $f$ equals 1, and at other points, $f$ equals 0).  

Next, the question is whether to use deterministic or stochastic approach in defending fingerprinting.  Because stochastic approach does not directly defend fingerprinting, it is unnecessary to randomize environment-specific constant (such as browser version) and introduce deterministic distribution function, which adds overhead and causes compatibility issues. Therefore, we mainly adopt determinism to combat fingerprinting. 


%Because

%Now, consider a fingerprint-able output as a random variable 

%distribution

%stochastic boils down to determinism

%when to choose determinism

Theoretically, we could make a fully deterministic browser mitigating all the stochastic factors. However, for similar reasons, it is unnecessary to fix the value for a random variable especially when the variable has a deterministic distribution function. A simple example is that there is no need to get rid of the random number generator in the JavaScript $Math$ object.  That is, precisely, our approach is a {\it mostly deterministic browser where stochastic factors have a deterministic distribution function}, for short, deterministic browser. 

